ProxNLP: a primal-dual augmented Lagrangian solver for nonlinear programming in Robotics and beyond

Mathematical optimization is the workhorse behind several aspects of modern robotics and control. In these applications, the focus is on constrained optimization, and the ability to work on manifolds (such as the classical matrix Lie groups), along with a specific requirement for robustness and speed. In recent years, augmented Lagrangian methods have seen a resurgence due to their robustness and flexibility, their connections to (inexact) proximal-point methods, and their interoperability with Newton or semismooth Newton methods. In the sequel, we present primal-dual augmented Lagrangian method for inequality-constrained problems on manifolds, which we introduced in our recent work, as well as an efficient C++ implementation suitable for use in robotics applications and beyond.

==> parts/mytemplate.tex <==

%% Define combination of Inria and LAAS colors

\definecolor{bluecolor}{rgb}{0.4,0.5,1}
\definecolor{bleuLAAS}{rgb}{0.18,0.35,0.55}
\definecolor{orangeLAAS}{RGB}{255,184,0}
\definecolor{rougeLAAS}{RGB}{197,50,83}

\definecolor{orangeinria}{RGB}{227,55,41} % Orange INRIA

\newcommand{\mytitle}[1]{
    {\small\color{bleuLAAS}LAAS/Inria DDP Reading group:} \\%
    #1
}

\defbeamertemplatealias{itemize item}{triangle}{default}
\setbeamertemplate{itemize item}[default]

